When Do Curricula Work in Federated Learning?

An oft-cited open problem of federated learning is the existence of data heterogeneity at the clients. One pathway to understanding the drastic accuracy drop in federated learning is by scrutinizing the behavior of the clients' deep models on data with different levels of "difficulty", which has been left unaddressed. In this paper, we investigate a different and rarely studied dimension of FL: ordered learning. Specifically, we aim to investigate how ordered learning principles can contribute to alleviating the heterogeneity effects in FL. We present theoretical analysis and conduct extensive empirical studies on the efficacy of orderings spanning three kinds of learning: curriculum, anti-curriculum, and random curriculum. We find that curriculum learning largely alleviates non-IIDness. Interestingly, the more disparate the data distributions across clients the more they benefit from ordered learning. We provide analysis explaining this phenomenon, specifically indicating how curriculum training appears to make the objective landscape progressively less convex, suggesting fast converging iterations at the beginning of the training procedure. We derive quantitative results of convergence for both convex and nonconvex objectives by modeling the curriculum training on federated devices as local SGD with locally biased stochastic gradients. Also, inspired by ordered learning, we propose a novel client selection technique that benefits from the real-world disparity in the clients. Our proposed approach to client selection has a synergic effect when applied together with ordered learning in FL.

==> Analysis.tex <==
\section{Analysis}


==> Broader-impact.tex <==
\section{Broader Impact and Limitation}\label{broader-impact}


The contributions of this paper expand the accuracy and applicability of federated learning into settings where either the difficulty among the data points at the particular client is not consistent or there is heterogeneity among the clients participating in the federation.

The practical impact of these results is that (a) clients/hospitals whose imaging dataset is generated by their in-house imaging systems can still benefit from client curriculum due to the inconsistent nature of the participants' data, even though their benefit from data curriculum is marginal due to the intra-data consistency. b) Better performance can be obtained in classification applications if the FL system takes advantage of the synergistic effect of the combination of client curriculum and data curriculum.


However, compared to the vanilla baseline, ordered learning in FL will increase small computation overhead caused by the inference (for scoring), as the scoring is a dynamic process and is done by the clients.


Our analyses further pave the road for future research directions. For instance, the impact of using CL on various image tasks in FL, such as segmentation or video action recognition tasks, can be explored in future works as they have their own specifications.


% There are many ways these advances can be put to a positive societal use. For instance, the approach can be used to classify medical images for rare illnesses, or illnesses where insufficient training data is available. Interestingly, COVID-19 at the time of the submission of this paper falls into this category in the United States. As part of our ongoing work to apply our research to practical applications, we found that as of June 2020, the COVIDx dataset~\cite{wang2020covid} is currently the largest accessible repository of COVID imaging in the US. This dataset contains 76 radiography images from 53 COVID-19 patient cases. Despite the prevalence of the illness, classifying these by severity maps them exactly into the few shot learning scenarios considered in this paper. 

% Naturally, any AI image classification technology can be put to negative use, for instance by repressive regimes improving their surveillance systems. 




% In the real world, the distributed dataset used in FL is often generated in-situ by clients, and the data is measured/generated using a particular sensor belonging to the client. For example, consider the case of a distributed image dataset generated by smartphone users using the onboard camera or a distributed medical imaging dataset generated by hospitals with their in-house imaging systems. In such scenarios, as there is a huge variety in the make and quality of the imaging sensors, the data generated by the clients is uniquely biased by the idiosyncrasies of the sensor, such as the noise, distortions, quality, etc. This introduces variability in the quality of the data at clients, in addition to the Non-IID nature of the data. However, it is interesting to note that these effects apply consistently across all the data at the specific client.

% From a curriculum point of view, as the data points are scored and ordered by difficulty, which is just a function of the loss value of that data point, these idiosyncratic distortions uniformly affect the loss/difficulty value of all the data at that particular client. Also, it is possible that the difficulty among the data points at the particular client is fairly consistent as the level of noise, quality of the sensor, etc. are the same across the data points. This bias in difficulty varies between clients but is often constant within the same client. Naturally, this introduces a \underline{heterogeneity in the clients} participating in the federation. In general, this can be thought of as some clients being "easy" and some being "difficult". \emph{ We can quantify this notion of consistency in difficulty by the standard deviation in the score of the data points at the client.}
 



==> Draft-CIFAR100.tex <==
% \subsection{Curriculum on clients}

\section{CIFAR-100}

\begin{table}[htbp]  % table 4n
\caption{Accuracy on CIFAR-100.  Arch = ResNet-9.}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & pacing & scoring & Non-IIDness & Curriculum & Anti & Random  & Vanilla \\
\midrule
FedAvg       & $Lin(0.8,0.2)$    & G-Loss   & Dir($\beta = 0.05$)   & $xxx$ & $xxx$ & $xxx$ & $26.43 \pm 0.77$ \\
\midrule

FedAvg      & $Lin(0.8,0.2)$    & G-Loss   & Dir($\beta = 0.2$)    & $xxx$ & $xxx$ & $xxx$ & $41.86 \pm 0.22$ \\
\midrule

FedAvg       & $Lin(0.8,0.2)$    & G-Loss   & Dir($\beta = 0.9$)    & $xxx$ & $xxx$ & $xxx$ & $48.14 \pm 0.22$ \\
\midrule


FedAvg      & $Lin(0.8,0.2)$    & G-Loss   & \#label2              & $xxx$ & $xxx$ & $xxx$ & $30.14 \pm 0.20$ \\
\midrule
FedAvg      & $Lin(0.8,0.2)$    & G-Loss   & IID             & $xxx$ & $xxx$ & $xxx$ & $49.32 \pm 0.14$ \\

\bottomrule
\end{tabular}
}
\end{table}



\begin{table}[htbp]  % table 8
\caption{Accuracy on CIFAR-100 for NIID-(20\%). Settings: $\mathit{rounds} = 100$, $\mathit{clients} = 100$, $\mathit{local\_epoch} = 10$, $\mathit{bs} = 10$, $\mathit{lr} = 0.01$, $\mathit{momentum} = 0.9$, Arch = ResNet-9.}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & pacing-f & pacing-a & pacing-b & scoring & Curriculum & Anti-Curriculum & Random Curriculum & Vanilla \\
% \midrule


% FedAvg & Linear    & 0.8  & 0.0025 & G-Loss & $51.15 \pm  1.38$ & $47.73 \pm  0.34$ & $51.11 \pm  0.12$ & $52.10 \pm  0.97$\\
       
% FedAvg & Linear    & 0.8  & 0.2    & G-Loss & $51.50 \pm  0.37$ & $48.15 \pm  0.38$ & $52.07 \pm  0.54$\\

\midrule

FedAvg  & Linear    & 0.8  & 0.0025 & G-Loss & $51.70 \pm  0.65$ & $47.77 \pm  1.42$ & $51.76 \pm  0.87$ & $51.50 \pm  0.53$\\

FedAvg  & Linear    & 0.8  & 0.2    & G-Loss & $52.13 \pm  0.93$ & $48.83 \pm  0.83$ & $52.24 \pm  0.17$ & \\

\midrule




FedAvg & Linear    & 0.8  & 0.0025 & LG-Loss & $52.47 \pm  0.24$ & $48.71 \pm  0.52$ & $50.37 \pm  0.79$ & \\


FedAvg & Linear    & 0.8  & 0.2    & LG-Loss & $53.37 \pm  0.83$ & $49.30 \pm  0.52$ & $51.73 \pm  1.03$ &\\

\midrule



FedAvg & Linear    & 0.8  & 0.0025 & LG-Pred & $49.87 \pm  1.81$ & $49.71 \pm  0.54$ & $50.72 \pm  0.64$ & \\
       
FedAvg & Linear    & 0.8  & 0.2    & LG-Pred & $51.18 \pm  0.09$ & $50.07 \pm  0.76$ & $50.93 \pm  0.24$ & \\

\midrule


 Avgerage & -- & -- & -- & -- & -- & -- & -- & XX  \\



\bottomrule
\end{tabular}
}
\end{table}





\vspace{2cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}[htbp]  % table ?
\caption{Accuracy on CIFAR-100 for NIID-(20\%). Settings: $\mathit{rounds} = 100$, $\mathit{clients} = 100$, $\mathit{local\_epoch} = 10$, $\mathit{bs} = 10$, $\mathit{lr} = 0.01$, $\mathit{momentum} = 0.9$, Arch = ResNet-9.}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & pacing-f & pacing-a & pacing-b & scoring & Curriculum & Anti-Curriculum & Random Curriculum & Vanilla \\
% \midrule


% FedAvg & Linear    & 0.8  & 0.0025 & LG-Loss & $51.33 \pm  0.48$ & $47.45 \pm  1.23$ & $51.22 \pm  1.15$ & $52.10 \pm  0.97$\\
       
% FedAvg & Linear    & 0.8  & 0.2    & LG-Loss & $52.18 \pm  0.30$ & $47.35 \pm  0.41$ & $51.75 \pm  0.65$\\

\midrule

FedAvg & Linear    & 0.8  & 0.0025 & LG-Loss & $52.47 \pm  0.24$ & $48.71 \pm  0.52$ & $50.37 \pm  0.79$ & $XX$\\


FedAvg & Linear    & 0.8  & 0.2    & LG-Loss & $53.37 \pm  0.83$ & $49.30 \pm  0.52$ & $51.73 \pm  1.03$ & $XX$\\

\midrule

 Avgerage & -- & -- & -- & -- & -- & -- & -- & --   \\



\bottomrule
\end{tabular}
}
\end{table}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\vspace{-2mm}
\begin{table}[htbp]  % table 9
\caption{Accuracy on CIFAR-100 for Dir(0.1). Settings: $\mathit{rounds} = 100$, $\mathit{clients} = 100$, $\mathit{local\_epoch} = 10$, $\mathit{bs} = 10$, $\mathit{lr} = 0.01$, $\mathit{momentum} = 0.9$, Arch = ResNet-9.}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & pacing-f & pacing-a & pacing-b & scoring & Curriculum & Anti-Curriculum & Random Curriculum & Vanilla \\

\midrule    

FedAvg  & Linear    & 0.8  & 0.0025 & G-Loss & $50.70 \pm  0.19$ & $47.93 \pm  0.56$ & $49.60 \pm  0.94$ & $50.17 \pm  0.46$\\


FedAvg  & Linear    & 0.8  & 0.2    & G-Loss & $51.54 \pm  0.35$ & $47.39 \pm  0.72$ & $51.52 \pm  0.20$ & \\

\midrule


FedAvg & Linear    & 0.8  & 0.0025 & LG-Loss & $50.42 \pm  0.19$ & $47.00 \pm  1.01$ & $50.31 \pm  1.25$ & \\
       
FedAvg & Linear    & 0.8  & 0.2    & LG-Loss & $51.34 \pm  1.18$ & $48.86 \pm  0.75$ & $50.46 \pm  0.56$\\

\midrule

FedAvg & Linear    & 0.8  & 0.0025 & LG-Pred & $50.92 \pm  0.36$ & $49.94 \pm  0.38$ & $50.38 \pm  0.84$ & \\
       
FedAvg & Linear    & 0.8  & 0.2    & LG-Pred & $50.18 \pm  1.09$ & $50.10 \pm  0.41$ & $51.17 \pm  0.67$ & \\

\midrule
    


 Avgerage & -- & -- & -- & -- & -- & -- & -- & $50.17 \pm  0.46$  \\


\bottomrule
\end{tabular}
}
\end{table}

\vspace{2cm}




==> Easy-Dataset.tex <==



\begin{figure*}[htbp]
\centering

\begin{subfigure}{0.23\linewidth}
    \includegraphics[width=1\linewidth]{figures/fmnist_lenet-5_linear0.8-0.2_gloss_fedavg_non-iidness_line.eps}
    % \caption{\scriptsize Linear}
    % \label{fig:purified_asr}
\end{subfigure}
\begin{subfigure}{0.23\linewidth}
    \includegraphics[width=1\linewidth]{figures/fmnist_lenet-5_linear0.8-0.2_gloss_fedprox_non-iidness_line.eps}
    % \caption{\scriptsize Step}
    % \label{fig:purified_asr}
\end{subfigure}
% \begin{subfigure}{0.24\linewidth}
%     \includegraphics[width=1\linewidth]{figures/table_03_log.eps}
%     \caption{\scriptsize table-03-log}
%     \label{fig:purified_asr}
% \end{subfigure}
\begin{subfigure}{0.23\linewidth}
    \includegraphics[width=1\linewidth]{figures/fmnist_lenet-5_linear0.8-0.2_gloss_scaffold_non-iidness_line.eps}
    % \caption{\scriptsize Quad}
    % \label{fig:purified_asr}
\end{subfigure}
\begin{subfigure}{0.23\linewidth}
    \includegraphics[width=1\linewidth]{figures/fmnist_lenet-5_linear0.8-0.2_gloss_scaffold_non-iidness_line.eps}
    % \caption{\scriptsize Exp}
    % \label{fig:purified_asr}
\end{subfigure}
\vspace{-3mm}
\caption{\footnotesize \textbf{Curriculum learning provide little benefit for different levels of data heterogeneity on easy datasets like FMNIST.} Test accuracy of different baselines when sweeping from 
extremely Non-IID setting, Dir (0.05) to highly IID setting, Dir(0.9). For each baseline, the average of final global test
accuracy is reported. We run each baseline 3 times
for 100 communication rounds with 10 local epochs. The figures from left to right, are for FedAvg, Fedprox, FedNova, and Scaffold baselines.}
\label{fig:fmnist-niid}

\end{figure*}




\section{Popular but easy datasets}\label{easy-dataset}
In the previous section, we perceived statistically significant benefits from ordered learning when the clients train on CIFAR-10 and CIFAR-100 which are considered medium- to-hard datasets in the FL context. Since many of the SOTA FL papers tested their algorithms on easy datasets, including MNIST~\cite{Ghosh-federated-2020, Vahidian-federated-2021}, FMNIST~\cite{vahidian-pacfl-2022,}, and similar families of datasets, for the sake of comprehensiveness, we also investigated the effect of ordered learning on one of these big families of datasets. The results on FMNIST for FedAvg, Fedprox, Scaffold, and Fednova are given in Fig.\ref{fig:fmnist-niid}. As is evident from the figure, curriculum learning has only marginal benefits for all of these baselines when trained on the FMNIST benchmark dataset. We dug deeper into the various training stages, from the initial communication round to the convergence, and found no benefit for ordered learning, whether the training time was short or long.





% Scaffold on FMNIST: Curr is better than anti, random, vanilla only in extreme Non-IID Dir(0.05) in low training.\\

% FedAvg on FMNIST:  there is no benefit in using ordered learning for fedavg for all cases high/low non-iid, low/high training.\\

% FedProx on FMNIST: there is no benefit in using ordered learning for fedprox for all cases high/low non-iid, low/high training.

\SV{Sreevatsank should show some visualizations about the scores of samples of FMNIST to show how these scores are close to each other which justifies why FMNIST does not benefit from ordered learning.}





\iffalse


\begin{table}[htbp]  % table 4n
\caption{FMNIST, Arch = LeNet-5,  $Linear(0.8,0.2)$, scoring=G-Loss}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & Non-IIDness & Curriculum & Anti & Random  & Vanilla \\
\midrule
FedAvg      & Dir($\beta = 0.05$)   & $80.06 \pm 0.48$ & $74.60 \pm 0.92$ & $80.45 \pm 0.56$ & $80.34 \pm 1.28$ \\
\midrule

FedAvg      & Dir($\beta = 0.2$)    & $85.12 \pm 0.57$ & $83.72 \pm 0.88$ & $86.12 \pm 0.62$ & $85.97 \pm 0.31$ \\
\midrule

FedAvg      & Dir($\beta = 0.9$)    & $87.23 \pm 0.03$ & $86.90 \pm 0.26$ & $88.10 \pm 0.10$ & $88.14 \pm 0.36$ \\


\bottomrule
\end{tabular}
}
\end{table}



\begin{table}[htbp]  % table 4n
\caption{FMNIST, Arch = LeNet,  $Linear(0.8,0.2)$, scoring=G-Loss}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & Non-IIDness & Curriculum & Anti & Random  & Vanilla \\
\midrule
FedProx     & Dir($\beta = 0.05$)   & $79.48 \pm 1.35$ & $74.29 \pm 2.39$ & $78.76 \pm 2.09$ & $80.97 \pm 1.56$ \\
\midrule

FedProx     & Dir($\beta = 0.2$)    & $84.99 \pm 0.06$ & $83.64 \pm 1.04$ & $86.01 \pm 0.21$ & $85.65 \pm 0.50$ \\
\midrule

FedProx     & Dir($\beta = 0.9$)    & $87.26 \pm 0.16$ & $87.10 \pm 0.15$ & $88.01 \pm 0.08$ & $87.95 \pm 0.21$ \\


\bottomrule
\end{tabular}
}
\end{table}


\begin{table}[htbp]  % table 4n
\caption{FMNIST, Arch = LeNet,  $Linear(0.8,0.2)$, scoring=G-Loss}.
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & Non-IIDness & Curriculum & Anti & Random  & Vanilla \\
\midrule
SCAFFOLD    & Dir($\beta = 0.05$)   & $81.26 \pm 1.21$ & $66.91 \pm 2.41$ & $79.78 \pm 1.33$ & $78.56 \pm 2.26$ \\
\midrule

SCAFFOLD    & Dir($\beta = 0.2$)    & $86.73 \pm 0.58$ & $83.80 \pm 0.13$ & $85.87 \pm 0.27$ & $86.01 \pm 0.13$ \\
\midrule

SCAFFOLD    & Dir($\beta = 0.9$)    & $88.49 \pm 0.07$ & $86.03 \pm 0.20$ & $87.92 \pm 0.22$ & $87.75 \pm 0.19$ \\


\bottomrule
\end{tabular}
}
\end{table}


\begin{table}[htbp]  % table 4n
\caption{FMNIST, Arch = LeNet,  $Linear(0.8,0.2)$, scoring=G-Loss}.
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule % Avg Final Local Acc
Algorithm & Non-IIDness & Curriculum & Anti & Random  & Vanilla \\
\midrule
FedNova     & Dir($\beta = 0.05$)   & $xxxx$ & $xxxx$ & $xxxx$ & $xxxxx$ \\
\midrule

FedNova      & Dir($\beta = 0.2$)     & $xxxx$ & $xxxx$ & $xxxx$ & $xxxxx$ \\
\midrule

FedNova      & Dir($\beta = 0.9$)     & $xxxx$ & $xxxx$ & $xxxx$ & $xxxxx$ \\


\bottomrule
\end{tabular}
}
\end{table}

\fi









==> Tables-of-Results.tex <==




\section{Tables of Results}

\subsection{Tables of scoring function}

\vspace{-2mm}
\begin{table}[H]  % table 3n
\caption{\scriptsize Evaluating the effect of using different scoring method on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-10 with IID data. All curricula use the linear pacing functions with $a = 0.8$ and $b = 0.2$. The results of vanilla FedAvg for this experiment is $51.81 \pm 1.83$.}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & Scoring & Curriculum & Anti & Random\\ % & Vanilla \\
\midrule
FedAvg        & $s_G$    & $56.15 \pm 0.58$ & $44.78 \pm 0.22$ & $51.23 \pm 0.33$ \\% & $52.73 \pm 0.53$ \\
\midrule
FedAvg         & $s_L$    & $56.33 \pm 0.43$ & $50.13 \pm 1.93$ & $52.89 \pm 0.89$ \\% & $52.19 \pm 1.65$ \\
\midrule
% FedAvg          & $s_{LG}$   & $56.00 \pm 0.38$ & $45.45 \pm 1.56$ & $52.22 \pm 0.35$ \\% & $53.37 \pm 0.76$ \\
% \midrule
FedAvg         & $s_{G}^{pred}$    & $54.56 \pm 0.86$ & $47.78 \pm 1.44$ & $50.88 \pm 0.56$ \\% & $51.34 \pm 1.09$ \\
\midrule
FedAvg        & $s_{L}^{pred}$   & $50.90 \pm 2.40$ & $49.53 \pm 0.56$ & $50.46 \pm 0.39$ \\% & $51.81 \pm 1.83$ \\
\midrule
FedAvg        & $s_{LG}^{pred}$   & $54.73 \pm 0.83$ & $48.65 \pm 0.82$ & $51.83 \pm 0.28$ \\% & $51.86 \pm 0.65$ \\
\bottomrule
\end{tabular}
}
\label{scoring-iid}
\end{table}






\vspace{-2mm}
\begin{table}[htbp]  % table 3n
\caption{\scriptsize Evaluating the effect of using different scoring method on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-10 with Non-IID (2) data. All curricula use the linear pacing functions with $a = 0.8$ and $b = 0.2$. Vanilla FedAvg is $40.75 \pm 0.59$. }
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & Scoring & Curriculum & Anti & Random \\%  & Vanilla \\
\midrule
FedAvg      & $s_G$            & $47.55 \pm 1.19$ & $34.24 \pm 0.54$ & $40.57 \pm 1.07$\\% & $40.75 \pm 0.59$ \\
\midrule
FedAvg      & $s_L$            & $43.16 \pm 0.41$ & $41.58 \pm 1.51$ & $41.90 \pm 0.75$\\% & $42.36 \pm 0.97$ \\
\midrule
% FedAvg      & $s_{LG}$         & $47.67 \pm 1.92$ & $35.76 \pm 0.37$ & $42.55 \pm 0.52$ \\%& $41.88 \pm 1.05$ \\
% \midrule
FedAvg      & $s_{G}^{pred}$   & $46.75 \pm 0.23$ & $40.09 \pm 1.66$ & $42.47 \pm 1.27$ \\%& $41.55 \pm 0.73$ \\
\midrule
FedAvg      & $s_{L}^{pred}$   & $41.22 \pm 1.97$ & $44.12 \pm 0.70$ & $41.35 \pm 0.40$ \\%& $42.15 \pm 1.58$ \\
\midrule
FedAvg      & $s_{LG}^{pred}$  & $46.66 \pm 1.12$ & $38.06 \pm 2.03$ & $43.34 \pm 0.33$ \\%& $41.48 \pm 1.73$ \\
\bottomrule
\end{tabular}
}
\label{scoring-niid}
\end{table}





\iffalse

\vspace{-2mm}
\begin{table}[H]  % table 3n
\caption{\scriptsize Evaluating the effect of using different scoring method on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-100 with IID data. All curricula use the linear pacing functions with $a = 0.8$ and $b = 0.2$. The results of vanilla FedAvg for this experiment is $51.81 \pm 1.83$. \SV{according to the results of cifar100, I'll decide to if we will fill the following table for FedAvg or Fedprox.}}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & Scoring & Curriculum & Anti & Random\\ % & Vanilla \\
\midrule
FedAvg        & $s_G$    & $xxx$ & $xxxx$ & $xxxx$ \\%
\midrule
FedAvg         & $s_L$    &$xxx$ & $xxxx$ & $xxxx$ \\%
\midrule
% FedAvg          & $s_{LG}$   & $xxx$ & $xxxx$ & $xxxx$ \\%
% \midrule
FedAvg         & $s_{G}^{pred}$    & $xxx$ & $xxxx$ & $xxxx$ \\%
\midrule
FedAvg        & $s_{L}^{pred}$   & $xxx$ & $xxxx$ & $xxxx$ \\%
\midrule
FedAvg        & $s_{LG}^{pred}$   & $xxx$ & $xxxx$ & $xxxx$ \\%
\bottomrule
\end{tabular}
}
\label{scoring-iid-cifar100}
\end{table}




\vspace{-2mm}
\begin{table}[H]  % table 3n
\caption{\scriptsize Evaluating the effect of using different scoring method on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-100 with Dir (0.05) data. All curricula use the linear pacing functions with $a = 0.8$ and $b = 0.2$. The results of vanilla FedAvg for this experiment is $51.81 \pm 1.83$.\SV{according to the results of cifar100, I'll decide to if we will fill the following table for FedAvg or Fedprox.}}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & Scoring & Curriculum & Anti & Random\\ % & Vanilla \\
\midrule
FedAvg        & $s_G$    & $xxx$ & $xxxx$ & $xxxx$ \\%
\midrule
FedAvg         & $s_L$    &$xxx$ & $xxxx$ & $xxxx$ \\%
\midrule
% FedAvg          & $s_{LG}$   & $xxx$ & $xxxx$ & $xxxx$ \\%
% \midrule
FedAvg         & $s_{G}^{pred}$    & $xxx$ & $xxxx$ & $xxxx$ \\%
\midrule
FedAvg        & $s_{L}^{pred}$   & $xxx$ & $xxxx$ & $xxxx$ \\%
\midrule
FedAvg        & $s_{LG}^{pred}$   & $xxx$ & $xxxx$ & $xxxx$ \\%
\bottomrule
\end{tabular}
}
\label{scoring-dir-cifar100}
\end{table}


\fi











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tables of pacing function}
The tables of pacing functions are 
\begin{table}[htbp]  % table 1n

\caption{\scriptsize Evaluating the effect of using different pacing function families and their hyperparameters on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-10 with IID data. The results of vanilla FedAvg for this experiment is $52.39 \pm 0.91$.}


\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & pacing-f & pacing-a & pacing-b & scoring & Curriculum & Anti & Random   \\
\midrule
            &         & 0.1  &        & G-Loss & $54.05 \pm 0.80$ & $50.21 \pm 1.02$ & $54.04 \pm 0.96$  \\
FedAvg      & Linear  & 0.5  & 0.2    & G-Loss & $54.92 \pm 1.01$ & $46.22 \pm 0.11$ & $52.38 \pm 1.12$    \\
            &         & 0.8  &        & G-Loss & $56.10 \pm 0.91$ & $44.44 \pm 0.75$ & $50.50 \pm 0.29$  \\
\midrule                                                            
            &         & 0.1  &        & G-Loss & $53.31 \pm 1.00$ & $50.64 \pm 0.45$ & $53.03 \pm 0.39$  \\
FedAvg      & Step    & 0.5  & 0.2    & G-Loss & $54.40 \pm 1.26$ & $46.38 \pm 1.32$ & $50.06 \pm 0.84$  \\
            &         & 0.8  &        & G-Loss & $55.54 \pm 1.87$ & $41.51 \pm 0.78$ & $46.54 \pm 0.87$  \\
\midrule                                                                    
            % &         & 0.1  &        & G-Loss & $52.69 \pm 1.10$ & $49.17 \pm 0.65$ & $51.85 \pm 0.36$  \\
% FedAvg      & Log     & 0.5  & 0.2    & G-Loss & $53.71 \pm 0.70$ & $48.81 \pm 0.96$ & $51.64 \pm 1.15$   \\
%             &         & 0.8  &        & G-Loss & $54.21 \pm 0.30$ & $48.30 \pm 0.50$ & $51.61 \pm 0.39$  \\
% \midjanrule                                
            &         & 0.1  &        & G-Loss & $53.58 \pm 0.76$ & $48.75 \pm 0.88$ & $52.71 \pm 1.52$  \\
FedAvg      & Quad    & 0.5  & 0.2    & G-Loss & $55.31 \pm 0.45$ & $47.11 \pm 1.65$ & $52.47 \pm 1.59$   \\
            &         & 0.8  &        & G-Loss & $56.36 \pm 0.41$ & $44.27 \pm 1.27$ & $51.05 \pm 0.14$  \\
\midrule                                
            &         & 0.1  &        & G-Loss & $51.84 \pm 0.96$ & $48.89 \pm 1.07$ & $51.73 \pm 0.81$   \\
FedAvg      & Exp     & 0.5  & 0.2    & G-Loss & $55.28 \pm 2.58$ & $45.82 \pm 1.31$ & $50.49 \pm 1.39$   \\
            &         & 0.8  &        & G-Loss & $57.45 \pm 1.48$ & $43.48 \pm 1.20$ & $49.90 \pm 1.10$   \\
\midrule                                                                
            &         & 0.1  &        & G-Loss & $53.76 \pm 1.64$ & $50.38 \pm 1.19$ & $52.98 \pm 0.99$   \\
FedAvg      & Sqrt    & 0.5  & 0.2    & G-Loss & $55.15 \pm 0.60$ & $47.92 \pm 1.38$ & $53.39 \pm 1.38$  \\
            &         & 0.8  &        & G-Loss & $54.84 \pm 0.75$ & $44.72 \pm 0.50$ & $50.37 \pm 1.17$   \\


% \cmidrule(lr{1em}){4-9} % make row divider on certain column
\bottomrule
\end{tabular}
}
\label{pacing-f-a}
\end{table}
% \clearpage



\vspace{-2mm}
\begin{table}[H]  % table 1n


\caption{\scriptsize Evaluating the effect of using different pacing function families and their hyperparameters on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-10 with Dir (0.05) data. The results of vanilla FedAvg for this experiment is $42.60 \pm 2.24$.}



\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & pacing-f & pacing-a & pacing-b & scoring & Curriculum & Anti & Random   \\
\midrule
            &        & 0.1  &        & G-Loss & $45.23 \pm 0.16$ & $37.16 \pm 2.44$ & $42.77 \pm 1.11$  \\
FedAvg      & Linear & 0.5  & 0.2    & G-Loss & $46.51 \pm 0.68$ & $33.84 \pm 0.38$ & $41.80 \pm 0.83$  \\
            &        & 0.8  &        & G-Loss & $47.01 \pm 1.26$ & $35.04 \pm 1.59$ & $40.97 \pm 1.16$  \\
\midrule                                                            
            &        & 0.1  &        & G-Loss & $43.54 \pm 0.70$ & $36.64 \pm 1.72$ & $42.68 \pm 1.72$  \\
FedAvg      & Step   & 0.5  & 0.2    & G-Loss & $45.61 \pm 0.49$ & $36.33 \pm 0.95$ & $41.56 \pm 0.74$  \\
            &        & 0.8  &        & G-Loss & $43.66 \pm 0.16$ & $31.25 \pm 1.92$ & $41.30 \pm 0.78$  \\
\midrule                                                                    

            &        & 0.1  &        & G-Loss & $45.73 \pm 0.72$ & $34.16 \pm 0.78$ & $41.64 \pm 0.96$  \\
FedAvg      & Quad   & 0.5  & 0.2    & G-Loss & $46.87 \pm 1.41$ & $34.20 \pm 0.60$ & $41.69 \pm 0.72$  \\
            &        & 0.8  &        & G-Loss & $46.81 \pm 0.23$ & $34.36 \pm 0.50$ & $40.11 \pm 0.93$  \\
\midrule                                
            &        & 0.1  &        & G-Loss & $44.63 \pm 1.25$ & $34.39 \pm 1.23$ & $40.88 \pm 1.71$  \\
FedAvg      & Exp    & 0.5  & 0.2    & G-Loss & $47.17 \pm 0.31$ & $36.99 \pm 0.96$ & $41.26 \pm 1.03$  \\
            &        & 0.8  &        & G-Loss & $44.30 \pm 0.24$ & $32.36 \pm 1.77$ & $41.06 \pm 1.14$  \\
\midrule                                                                
            &        & 0.1  &        & G-Loss & $45.00 \pm 1.64$ & $37.31 \pm 0.16$ & $42.04 \pm 1.33$  \\
FedAvg      & Sqrt   & 0.5  & 0.2    & G-Loss & $45.91 \pm 0.61$ & $35.97 \pm 1.21$ & $41.70 \pm 1.36$  \\
            &        & 0.8  &        & G-Loss & $46.90 \pm 0.69$ & $34.03 \pm 1.24$ & $41.11 \pm 0.16$  \\


% \cmidrule(lr{1em}){4-9} % make row divider on certain column
\bottomrule
\end{tabular}
}
\label{pacing-f-a-cifar10-dir}
\end{table}
% \clearpage


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% $46.26 \pm  0.55$



\vspace{-2mm}
\begin{table}[htbp]  % table 2n
\caption{\scriptsize Evaluating the effect of  hyperparameter $b$ on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-10 with IID data. The results of vanilla FedAvg for this experiment is $55.32 \pm 0.78$. }
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & pacing-f & pacing-a & pacing-b & scoring & Curriculum & Anti & Random   \\
\midrule
            &         &      & 0.0025   & G-Loss & $57.88 \pm 0.11$ & $45.84 \pm 1.93$ & $52.52 \pm 0.64$  \\
            &         &      & 0.1      & G-Loss & $57.57 \pm 0.48$ & $46.50 \pm 0.24$ & $53.16 \pm 0.33$  \\
FedAvg      & Linear  & 0.8  & 0.2      & G-Loss & $57.71 \pm 0.21$ & $48.09 \pm 0.61$ & $53.53 \pm 0.52$  \\
            &         &      & 0.5      & G-Loss & $55.78 \pm 0.26$ & $50.81 \pm 0.76$ & $54.01 \pm 0.39$   \\
            &         &      & 0.8      & G-Loss & $55.89 \pm 0.36$ & $52.82 \pm 0.69$ & $54.71 \pm 0.33$   \\


% \cmidrule(lr{1em}){4-9} % make row divider on certain column
\bottomrule
\end{tabular}
}
\label{pacing-b}
\end{table}




\vspace{-2mm}
\begin{table}[H]  % table 2n
\caption{\scriptsize Evaluating the effect of  hyperparameter $b$ on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-10 with  Dir (0.05) data. The results of vanilla FedAvg for this experiment is $42.60 \pm 2.24$.}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & pacing-f & pacing-a & pacing-b & scoring & Curriculum & Anti & Random   \\
\midrule
            &         &      & 0.0025   & G-Loss & $45.95 \pm 0.15$ & $33.08 \pm 1.03$ & $42.72 \pm 1.12$  \\
            &         &      & 0.1      & G-Loss & $46.84 \pm 0.39$ & $30.47 \pm 2.11$ & $41.34 \pm 0.73$  \\
FedAvg      & Linear  & 0.8  & 0.2      & G-Loss & $47.07 \pm 0.86$ & $34.11 \pm 0.35$ & $41.07 \pm 0.70$  \\
            &         &      & 0.5      & G-Loss & $46.82 \pm 0.66$ & $37.64 \pm 1.07$ & $42.70 \pm 1.07$  \\
            &         &      & 0.8      & G-Loss & $44.21 \pm 0.28$ & $40.78 \pm 1.60$ & $43.08 \pm 0.75$  \\


% \cmidrule(lr{1em}){4-9} % make row divider on certain column
\bottomrule
\end{tabular}
}
\label{pacing-b-cifar10-dir}
\end{table}






\vspace{-2mm}
\begin{table}[H]  % table 1n


\caption{\scriptsize Evaluating the effect of using different pacing function families and their hyperparameters on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-100 with Dir (0.05) data. The results of vanilla FedAvg for this experiment is $xxxx$. \SV{Saeed-should include}}



\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & pacing-f & pacing-a & pacing-b & scoring & Curriculum & Anti & Random   \\
\midrule
            &         & 0.1  &        & G-Loss & $xx$ & $xx$ & $xx$  \\
FedAvg      & Linear  & 0.5  & 0.2    & G-Loss & $xx$ & $xx$ & $xx$  \\
            &         & 0.8  &        & G-Loss & $xx$ & $xx$ & $xx$  \\
\midrule
            &         & 0.1  &        & G-Loss & $xx$ & $xx$ & $xx$  \\
FedAvg      & Step    & 0.5  & 0.2    & G-Loss & $xx$ & $xx$ & $xx$  \\
            &         & 0.8  &        & G-Loss & $xx$ & $xx$ & $xx$  \\
\midrule
            &         & 0.1  &        & G-Loss & $xx$ & $xx$ & $xx$  \\
FedAvg      & Quad    & 0.5  & 0.2    & G-Loss & $xx$ & $xx$ & $xx$  \\
            &         & 0.8  &        & G-Loss & $xx$ & $xx$ & $xx$  \\
\midrule
            &         & 0.1  &        & G-Loss & $xx$ & $xx$ & $xx$  \\
FedAvg      & Exp     & 0.5  & 0.2    & G-Loss & $xx$ & $xx$ & $xx$  \\
            &         & 0.8  &        & G-Loss & $xx$ & $xx$ & $xx$  \\
\midrule
            &         & 0.1  &        & G-Loss & $xx$ & $xx$ & $xx$  \\
FedAvg      & Sqrt    & 0.5  & 0.2    & G-Loss & $xx$ & $xx$ & $xx$  \\
            &         & 0.8  &        & G-Loss & $xx$ & $xx$ & $xx$  \\


% \cmidrule(lr{1em}){4-9} % make row divider on certain column
\bottomrule
\end{tabular}
}
\label{pacing-f-a-cifar100}
\end{table}
% \clearpage





\vspace{-2mm}
\begin{table}[H]  % table 2n
\caption{\scriptsize Evaluating the effect of  hyperparameter $b$ on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-100 with  Dir (0.05) data. The results of vanilla FedAvg for this experiment is $xxxx$. (this is wrong one!!!!)}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & pacing-f & pacing-a & pacing-b & scoring & Curriculum & Anti & Random   \\
\midrule
            &         &      & 0.0025   & G-Loss & $47.49 \pm 0.16$ & $43.91 \pm 0.87$ & $46.74 \pm 1.26$  \\
            &         &      & 0.1      & G-Loss & $48.45 \pm 0.60$ & $44.89 \pm 0.47$ & $47.88 \pm 0.52$  \\
FedAvg      & Linear  & 0.8  & 0.2      & G-Loss & $48.11 \pm 0.53$ & $44.42 \pm 0.29$ & $47.85 \pm 0.66$  \\
            &         &      & 0.5      & G-Loss & $47.78 \pm 0.08$ & $44.58 \pm 0.38$ & $47.52 \pm 0.21$  \\
            &         &      & 0.8      & G-Loss & $47.10 \pm 0.29$ & $44.07 \pm 0.18$ & $46.83 \pm 0.77$  \\


% \cmidrule(lr{1em}){4-9} % make row divider on certain column
\bottomrule
\end{tabular}
}
\label{pacing-b-cifar100}
\end{table}





\vspace{-2mm}
\begin{table}[H]  % table 2n
\caption{\scriptsize Evaluating the effect of  hyperparameter $b$ on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-100 with  Dir (0.05) data. The results of vanilla FedAvg for this experiment is $48.11 \pm 0.38$.\SV{Saeed-should include} }
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm & pacing-f & pacing-a & pacing-b & scoring & Curriculum & Anti & Random   \\
\midrule
            &         &      & 0.0025   & G-Loss & $45.18 \pm 1.02$ & $39.81 \pm 0.60$ & $45.35 \pm 0.35$  \\
            &         &      & 0.1      & G-Loss & $46.91 \pm 0.80$ & $41.46 \pm 0.58$ & $46.43 \pm 0.58$  \\
FedAvg      & Linear  & 0.8  & 0.2      & G-Loss & $47.59 \pm 0.68$ & $43.17 \pm 0.63$ & $46.60 \pm 0.40$  \\
            &         &      & 0.5      & G-Loss & $47.99 \pm 0.25$ & $45.51 \pm 0.26$ & $47.16 \pm 0.45$  \\
            &         &      & 0.8      & G-Loss & $48.69 \pm 0.24$ & $47.27 \pm 0.26$ & $47.34 \pm 0.31$  \\


% \cmidrule(lr{1em}){4-9} % make row divider on certain column
\bottomrule
\end{tabular}
}
\label{pacing-b-cifar100}
\end{table}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tables of effect of num of partitions}



\vspace{-2mm}
\begin{table}[htbp]  % table Ptest
\caption{\scriptsize Evaluating the impact of the amount of data each client owns on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-10 with Non-IID (2) data. All curricula use the linear pacing functions with $a = 0.8$ and $b = 0.2$. Here lower partition corresponds to higher amount of data.\textbf{we should add one personalized algorithm as well and one dataset as well}}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm  & partitions & Curriculum & Anti & Random  & Vanilla \\
\midrule
FedAvg       & 100 & $47.23 \pm 0.23$ & $34.80 \pm 0.97$ & $42.93 \pm 2.13$ & $41.42 \pm 0.91$ \\
\midrule
FedAvg        & 200 & $44.22 \pm 0.58$ & $33.93 \pm 0.53$ & $40.33 \pm 0.80$ & $38.72 \pm 0.29$ \\
\midrule
FedAvg        & 400 & $41.13 \pm 0.78$ & $28.56 \pm 1.32$ & $35.93 \pm 1.21$ & $35.84 \pm 1.13$ \\
\midrule
FedAvg      & 800 & $35.96 \pm 1.78$ & $28.40 \pm 0.49$ & $31.80 \pm 1.13$ & $31.16 \pm 1.09$ \\

\bottomrule
\end{tabular}
}
\label{table:cifar10-noniid2-fedavg}
\end{table}



\iffalse
\vspace{-2mm}
\begin{table}[htbp]  % table Ptest
\caption{\scriptsize Evaluating the impact of the amount of data each client owns on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-10 with Dir(0.05) data. All curricula use the linear pacing functions with $a = 0.8$ and $b = 0.2$. Here lower partition corresponds to higher amount of data.\textbf{we should add one personalized algorithm as well and one dataset as well}}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm  & partitions & Curriculum & Anti & Random  & Vanilla \\
\midrule
FedAvg       & 100 & $xxx$ & $xxx$ & $xxx$ & $xxx$ \\
\midrule
FedAvg        & 200 &  $xxx$ & $xxx$ & $xxx$ & $xxx$ \\
\midrule
FedAvg        & 400 &  $xxx$ & $xxx$ & $xxx$ & $xxx$ \\
\midrule
FedAvg      & 800 &  $xxx$ & $xxx$ & $xxx$ & $xxx$ \\

\bottomrule
\end{tabular}
}
\end{table}
\fi





\begin{table}[H]  % table Ptest
\caption{\scriptsize Evaluating the impact of the amount of data each client owns on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-10 with Dir (0.5) data. All curricula use the linear pacing functions with $a = 0.8$ and $b = 0.2$. Here lower partition corresponds to higher amount of data.}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm  & partitions & Curriculum & Anti & Random  & Vanilla \\
\midrule
FedProx  & 100 & $54.52 \pm 0.98$ & $46.36 \pm 0.93$ & $50.92 \pm 1.07$ & $ 53.38 \pm 1.56 $ \\
\midrule
FedProx  & 200 & $49.98 \pm 0.58$ & $42.74 \pm 0.79$ & $47.30 \pm 1.03$ & $ 47.65 \pm 1.35 $ \\
\midrule
FedProx  & 400 & $47.94 \pm 0.96$ & $40.59 \pm 0.18$ & $43.34 \pm 0.97$ & $ 43.63 \pm 1.09 $ \\
\midrule
FedProx  & 800 & $44.31 \pm 0.52$ & $38.71 \pm 0.44$ & $40.85 \pm 0.53$ & $ 39.18 \pm 1.11 $ \\
\bottomrule
\end{tabular}
}
\label{table:cifar10-noniid2-fedprox}
\end{table}








\begin{table}[H]  % table Ptest
\caption{\scriptsize Evaluating the impact of the amount of data each client owns on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-10 with Dir (0.5) data. All curricula use the linear pacing functions with $a = 0.8$ and $b = 0.2$. Here lower partition corresponds to higher amount of data.}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm  & partitions & Curriculum & Anti & Random  & Vanilla \\
\midrule
FedAvg   & 100 & $55.43 \pm 0.38$ & $46.09 \pm 1.38$ & $50.96 \pm 1.54$ & $52.66 \pm 0.59$ \\
\midrule
FedAvg   & 200 & $50.20 \pm 0.18$ & $41.13 \pm 0.26$ & $47.53 \pm 0.35$ & $46.34 \pm 0.28$ \\
\midrule
FedAvg   & 400 & $45.63 \pm 1.81$ & $38.62 \pm 1.31$ & $42.67 \pm 0.47$ & $42.22 \pm 1.48$ \\
\midrule
FedAvg   & 800 & $41.98 \pm 0.74$ & $36.61 \pm 0.86$ & $39.75 \pm 0.93$ & $37.90 \pm 0.41$ \\
\bottomrule
\end{tabular}
}
\label{table:cifar10-noniid2-fedprox}
\end{table}








\begin{table}[H]  % table Ptest
\caption{\scriptsize Evaluating the impact of the amount of data each client owns on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-10 with Dir (0.05) data. All curricula use the linear pacing functions with $a = 0.8$ and $b = 0.2$. Here lower partition corresponds to higher amount of data.}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm  & partitions & Curriculum & Anti & Random  & Vanilla \\
\midrule
FedProx  & 100 & $46.73 \pm 0.83$ & $33.72 \pm 1.53$ & $40.84 \pm 0.62$ & $41.61 \pm 1.11$ \\
\midrule
FedProx  & 200 & $42.85 \pm 0.36$ & $31.90 \pm 0.76$ & $38.51 \pm 1.42$ & $37.58 \pm 0.52$ \\
\midrule
FedProx  & 400 & $39.99 \pm 0.98$ & $27.40 \pm 2.90$ & $35.05 \pm 0.33$ & $34.38 \pm 2.72$ \\
\midrule
FedProx  & 800 & $36.32 \pm 0.36$ & $28.12 \pm 2.13$ & $32.08 \pm 0.45$ & $30.58 \pm 1.03$ \\
\bottomrule
\end{tabular}
}
\label{table:cifar10-noniid2-fedprox}
\end{table}



\iffalse
\begin{table}[H]  % table Ptest
\caption{\scriptsize Evaluating the impact of the amount of data each client owns on the accuracy when the clients employ curriculum, anti-curriculum or random ordering during their local training on CIFAR-100 with Dir (0.05) data. All curricula use the linear pacing functions with $a = 0.8$ and $b = 0.2$. Here lower partition corresponds to higher amount of data.}
\vspace{-3mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
Algorithm  & partitions & Curriculum & Anti & Random  & Vanilla \\
\midrule
FedProx  & 100 & $xxx$ & $xxxx$ & $xxx$ & $xxx$ \\
\midrule
FedProx  & 200 & $xxx$ & $xxxx$ & $xxx$ & $xxx$ \\
\midrule
FedProx  & 400 & $xxx$ & $xxxx$ & $xxx$ & $xxx$ \\
\midrule
FedProx   & 800 & $xxx$ & $xxxx$ & $xxx$ & $xxx$ \\
\bottomrule
\end{tabular}
}
\label{table:cifar10-noniid2-fedprox}
\end{table}
\fi

==> curriculum-on-client.tex <==
 \vspace{-2mm}
 \section{Curriculum on Clients} \label{curr-on-client}
% % \section{When do curriculum not work in FL?}


%  Motivation of Curriculum on client ?
 
%  - Practical Federated Learning setting is In-situ 
 
A major appeal of federated learning is in its ability to enable training of a model in a decentralised manner, which obviates the need for collating the data into a centralized location. In the real-world, the distributed dataset used in federated learning is often generated in-situ by clients and the data is measured/generated using a particular sensor belonging to the client. For example, consider the case of a distributed image dataset generated by smartphone users using the onboard camera or a distributed medical imaging dataset generated by hospitals with their in-house imaging systems. In such scenarios, as there is a huge variety in the make and quality of the imaging sensors, the data generated by the clients is uniquely biased by the idiosyncrasies of the sensor, such as the noise, distortions, quality, etc. This introduces variability in the quality of the data at clients, in addition to the Non-IID nature of the data. However it is interesting to note that, these effects apply consistently across all the data at the specific client. 

From a curriculum point of view, as the data points are scored and ordered by difficulty, which is just a function of the loss value of that data point, these idiosyncratic distortions uniformly affect the loss/difficulty value of all the data at that particular client. Also, it is possible that the difficulty among the data points at the particular client is fairly consistent as the level of noise, quality of sensor, etc., are the same across the data points. This bias in difficulty varies between clients but is often constant within the same client. Naturally, this introduces a \underline{heterogeneity in the clients} participating in the federation. In general, this can be thought of as some clients being "easy" and some being "difficult". \emph{ We can quantify this notion of consistency in difficulty by the standard deviation in the score of the data points at the client.}
 
% Consider a real-world scenario of users that participate in federated learning, in which, the users bring along with them their locally stored data that is often sourced/generated/collected on the same device that participates in the federation. For example a smartphone camera device that brings along the photographs taken by the very same device for federation. As there is a huge diversity in the make and quality of smartphone cameras we have a wide spectrum of quality in images, also these devices/sensors could have idiosyncratic distortions and noise in the data they produce. This creates a heterogeneous user base with a wide gamut of data quality. Interestingly, as these effects apply consistent to all the data at a specific user, the relative quality of data is quite consistent in the local user dataset.  

% In the previous sections, we have studied the effects of curriculum in the Federated learning setting. In this section, we will look into certain federated learning scenarios in which curriculum does not work.

% The heterogeneity in the quality of the user datasets and their relative local consistency naturally translates into an ordering over the datasets (thereby users) of varying difficulty, the data of which is of relatively consistent difficulty. (Prove this). The difficulty of a a dataset/user is quantified by the mean of loss and the consistency is quantified by the variance of loss of the constituent data points. 

% Add figure with G-loss 

\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.3\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ClientCurr/DC_noeffect_iid_bar_E.eps}
         \caption{IID}
         \label{subfig:DC_noeffect_iid}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ClientCurr/DC_noeffect_dir02_bar_E.eps}
         \caption{Dir(0.2)}
         \label{subfig:DC_noeffect_dir02}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ClientCurr/Dc_noeffect_dir005_bar_E.eps}
         \caption{Dir(0.05)}
         \label{subfig:DC_noeffect_dir005}
     \end{subfigure}
    \vspace{-3mm}
\caption{\footnotesize \textbf{ Consistency in data difficulty at the client hurts efficacy of curricula.} The effect of consistency in the difficulty distribution at the client nullifies the effect of curricula. The standard deviation values of (Low, High) consistency for the IID is $(0.52,0.01)$, Dir(0.2) is $(0.51,0.14)$, Dir(0.05) is $(0.50,0.13)$. Note that we use Algorithm~\ref{alg:partiiton_diff_dist} to construct partitions with varying difficulty and as detailed in Section~\ref{sec:difficulty_based_partitioning} it is not possible to control the partition difficulty value with arbitrary precision and hence the above minor variations. The Low consistency scenario is generated using $f_{ord}=0.0$ and the high consistency scenario uses $f_{ord}=1.0$.}
\label{fig:DC_noeffect_E}
\end{figure}


\SV{we dont need to define a new terminology like positive curr. Especially when we are using it once. Lets stick to the standard terms.}
When the standard deviation of the intra-client data is low, i.e., the difficulty of the data within a client is consistent\SV{the previous sentence is not necessarily true}, we find that curriculum on federated learning behaves very differently in these kinds of scenarios. We observe the advantage of positive curriculum (refereed to by 'curr') diminish significantly and converging to a random curricula as shown in Fig~\ref{fig:DC_noeffect_E}. The advantage of curriculum can be defined as $A_{o} = accuracy(o) - accuracy(vanilla)$, where $o \in \{curr,anti,rand\}$. 

\subsection{Client Curriculum}

% Using Algorithm~\ref{alg:partiiton_diff_dist} with $f_{ord}=1$ we generate and study the effects

% It is interesting to note that, in a real-world FL scenarios the local consistency at the clients could be high, at the same time, the level of heterogeneity among clients is also higher. 

The technique of ordered learning that presented in previous sections is designed to exploit the heterogeneity of data at the clients, but, is not geared to effectively leverage the heterogeneity between the clients that naturally emerge in the real-world. Also, as we see in Fig~\ref{}, the benefits of the algorithm severely depend on the data at the client having a diverse set difficulties. 

% which is still a non-trivial and open problem because of the Given the large-scale distributed and heterogeneous nature of the training data.

In the literature, some recent works have dabbled with the idea of smarter clients selection, and many selection criteria have been suggested, such as, importance sampling, where the probabilities for clients to be selected is proportional to their importance measured by the norm of update~\cite{Optimal-Client-Sampling-2022}, test accuracy~\cite{client-selection-iot-2021}. The ~\cite{power-of-choice-2020} paper proposes client selection based on local loss where clients with higher loss are preferential selected to participate in more rounds of federation, which is in stark contrast to~\cite{client-selection-2022-curr} in which the clients with a lower loss are preferentially selected. It’s clear from the literature that the heterogeneous environment in federated learning can hamper the overall training and convergence speed~\cite{haddadpour2019convergence, mahdavi2020-APFL}, but the empirical observations on client selection criteria either are in conflict or their efficacy is minimal. In this work, inspired by curriculum learning, we try to propose a more sophisticated method of client selection that generalizes the above strategies to the FL setting. 

We propose to extend the ideas of curriculum onto the set of clients, in order to leverage the heterogeneity in the set of clients. To the best of our knowledge, our paper is the first attempt to introduce the idea of curriculum on clients in a FL setting. A lot of ideas of curricula can be neatly be extended to apply over the set of clients. We define a scoring function, a pacing function and an ordering for curricula on the set of clients. We define the client loss as the mean loss of the local data points at the client, and client score can be thought of as inversely proportional to loss.

\[
\mathcal{L}_k =\frac{1}{\|\mathbb{D}_m\|}\sum\limits_{j}^{\|\mathcbb{D}_m\|} l_j    \label{eq:client_loss}
\]

\noindent where $m$ is the index for client, $\mathbb{D}_m$ represents the dataset at client $m$, $l_j$ is the loss of $j$th data point in $\mathbb{D}_m$. The action of the pacing function here is to scale the participation rate of the clients in the federation.~\SV{we should explain the setting a bit more} The ordering is over the set of client scores.

Thereby we have two sets of curricula, one that acts locally on the client data and the other that acts on the set of clients. Henceforth we will refer to these as data curriculum and client curriculum respectively. We study the interplay of these curricula in detail in Section~\ref{sec:ablation_study}.


\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.3\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ClientCurr/CC_effect_iid_bar_E.eps}
         \caption{IID}
         \label{subfig:CC_effect_iid}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ClientCurr/CC_effect_dir02_bar_E.eps}
         \caption{Dir(0.2)}
         \label{subfig:CC_effect_dir02}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ClientCurr/CC_effect_dir005_bar_E.eps}
         \caption{Dir(0.05)}
         \label{subfig:CC_effect_dir005}
     \end{subfigure}
    \vspace{-3mm}
\caption{\footnotesize \textbf{Client curriculum does not suffer from low heterogeneity in the data difficulty and is effective when data curriculum is not.} The scenario shown here is the same high local consistency scenario from Fig~\ref{fig:DC_noeffect_E}. As we observe the client curriculum is able to overcome the limitations of the data curriculum.}
\label{fig:CC_effect_E}
\end{figure}

As shown in Fig~\ref{fig:CC_effect_E} we are able to realise an $A_{curr}$ \SV{should not be $A_{o}$?} of $5.67-7.19$\% for the different values of Non-IIDness using our proposed client curriculum algorithm in the scenario with high consistency in the client data where the data curriculum has reduced/no benefits. This illustrates that the client curriculum is able to effectively overcome the limiting constraint of local variability in data and is able to leverage the heterogeneity in the set of clients to its benefit.

\subsection{Difficulty based partitioning} \label{sec:difficulty_based_partitioning}

%  - Why use this technique? 
%  To be able to test the idea while also comparing to standard baselines

For the experiments in this section, we require client datasets ($\mathbb{D}_m$) of varying difficulty at the desired level of Non-IIDness. In order to construct partitions of varying difficulty, we need to address two key challenges, one, we need a way to accurately assess the difficulty of each of the data points, two, we need to be able to work with different levels of Non-IIDness.

In order to address the first challenge, we use an apriori trained expert model $\theta_{\mathcal{E}}$ which is trained on the entire baseline dataset and is of the same network topology as that of the global model, and use it for ranking the data points in the order of difficulty. As the expert model is of the same topology as that of the model that we intend to train, and that it is trained on the entire dataset it is an accurate judge of the difficulty of the data points. Interestingly, this idea can be extended to be used as a scoring method for curriculum as well. We call this scoring method called the expert scoring $s_{E}$. We look at this in greater detail in Section~\ref{}.

To the second challenge, a possible solution is to first partition the standard dataset into the desired non-IID partitions using well know techniques such as the Dirichlet distribution and followed by adding different levels of noise to the samples of the different data partitions. This would partitions with varying difficulty, however, doing so would alter the standard baseline dataset and we will loose the ability to compare the results to known baseline values and between different settings. We would like to be able to compare our performance results with standard baselines and hence we require a method that does not alter the data or resort to data augmentation techniques, and hence we devise a technique that does just that. 

Starting with the baseline dataset, we first partition it into the desired Non-IID partitions the same as before, but then instead of adding noise to the dataset we attempt to reshuffle the data among partitions in such a way that we create "easy" partitions and "hard" partitions. This can be achieved by ordering the data in an increasing order of difficulty and distribute the data among the partitions starting from the "easy" data points, all the while honoring the Non-IID class counts of each of the partitions as determined by the Non-IID distribution. The outline is detailed in Algorithm~\ref{alg:partiiton_diff_dist}.  

It is to be noted that, although we are able to generate partitions of varying difficulty we do not have direct control over the "difficulty" of each of the partitions and hence cannot generate partitions with arbitrary distribution of difficulty as can be done by adding noise.


\begin{algorithm}[H]
\caption{Partition Difficulty Distribution}\label{alg:partiiton_diff_dist}

\small
\begin{algorithmic}
\item \hspace{-6mm}
\noindent \colorbox[rgb]{1, 0.95, 1}{
\begin{minipage}{0.9\textwidth}
\textbf{Input:} partitions $\{\mathbb{P}_0,\mathbb{P}_1,...,\mathbb{P}_N\}$ of the input dataset $\mathbb{D}$ of $C$ classes indexed by $c$, fraction of each partition to replace $f_{ord}\in(0,1]$, expert model $\theta_{\mathcal{E}}$

\end{minipage}
}
\item \hspace{-6mm}
\colorbox[gray]{0.95}{
\begin{minipage}{0.9\textwidth}
\item  \textbf{Class prior of partitions and dataset:}


\item     \hspace*{\algorithmicindent} \textbf{for } each partition $i=0,1,2,...,N$ \textbf{do}
\item     \hspace*{\algorithmicindent} \quad $\mathbb{P}_i \leftarrow$ count(data points of class $c$ in partition $i$)
\item     \hspace*{\algorithmicindent}    
\item     \hspace*{\algorithmicindent} Compute loss ($\mathcal{L}$) for each data point in $\mathbb{D}$ using $\theta_{\mathcal{E}}$
\item     \hspace*{\algorithmicindent} $\mathbb{D}_{c} \leftarrow$ argsort($\mathcal{L}_c$)

\end{minipage}
}
\item \hspace{-6mm}
\colorbox[rgb]{0.95, 0.98, 1}{
\begin{minipage}{0.9\textwidth}

\item  \textbf{Reconstitute partition:}

% \item     \hspace*{\algorithmicindent} Obtain the score of each data sample using $\theta^{t}_g $:
% \hspace*{\algorithmicindent} \quad $s({\bf{x_i}}, y_i)=1/\mathcal{L}(f_{\theta^{t}_g}({\bf{x}}_i),y_i )$

\item     \hspace*{\algorithmicindent} $id_c = cumsum_i(N_{i,c})$
\item 
\item     \hspace*{\algorithmicindent} Distribute $f_{ord}$ 
\item     \hspace*{\algorithmicindent} \textbf{for } each partition $i=0,1,2,...,N$ \textbf{do}
\item     \hspace*{\algorithmicindent} \quad $\mathbb{P}_i \leftarrow \mathbb{P}_i \cup$ partition($f_{ord}*N_{i,c}$ elements of $\mathbb{D}_c$ beginning at $id_{i,c}$)
\item     \hspace*{\algorithmicindent} $\mathbb{D'}_c \leftarrow$ remaining elements of $\mathbb{D}_c$
\item 
\item     \hspace*{\algorithmicindent} Distribute remaining $(1-f_{ord})$
\item     \hspace*{\algorithmicindent} \textbf{for } each partition $i=0,1,2,...,N$ \textbf{do}
\item     \hspace*{\algorithmicindent} \quad $\mathbb{P}_i \leftarrow \mathbb{P}_i \cup$ random($(1-f_{ord})*N_{i,c}$ elements of $\mathbb{D'}_c$)


\end{minipage}
}
\end{algorithmic}
\end{algorithm}




% Our proposed idea looks to ﬁnd a sweet spot between fast convergence and heterogeneity by looking at smart clients selection and scheduling techniques.
 
% Our approach does not require any additional operation on the clients side, and can be seamlessly integrated in standard FL implementations.


% Current sampling approaches in FL are either biased, or non optimal in terms of server-clients communications and training stability. To overcome this issue, we introduce clustered sampling for clients selection.


% The above results demonstrate that the probing loss can be used as an indicator of client selection for better FL accuracy under non-IID setting.




% Using this insight, we propose the P OWER - OF - CHOICE client selection strategy and show by extensive experiments that P OWER - OF - CHOICE yields up to 3× faster convergence with $10\%$ higher test performance than the standard federated averaging with random selection. P OWER - OF - CHOICE is designed to incur minimal communication and computation overhead, enhancing resource efﬁciency in federated learning. In fact, we show that even with 3× less clients participating in each round as compared to random selection, P OWER - OF - CHOICE gives 2×

% Several works have analyzed the convergence of federated learning by accounting of data heterogeneity, communication and computation limitations, and partial client participation. However, they assume unbiased client participation, where clients are selected at random or in proportion of their data sizes.

% In this paper, we present the ﬁrst convergence analysis of federated optimization for biased client selection strategies, and quantify how the selection bias affects convergence speed.

% However, adaptive client selection that is cognizant of the training progress at each client has not been understood yet.


% We reveal that biasing client selection towards clients with higher local loss achieves faster error convergence.












% Some recent work looks to do client selection based on different criteria like higher potential for global model convergence or good network conditions. Cho et. al. [10] revealed that a selection biased towards clients with higher local loss can increase the speed of convergence. This is because higher loss indicates higher potential for model improvement. The proposed POWEROF-CHOICE algorithm can yield up to 3X faster convergence and 10% higher test accuracy compared with conventional federated learning with



% From Fig~\ref{} it can be noted that the efficacy of curriculum in the FL setting diminishes with the increasing consistency in the local data difficulty and it turns out to be completely ineffective for the $f_{ord} = 1$ scenario.


% As we also show in section~\ref{} that the heterogeneous environment completely negate benefits of curriculum learning.

\subsection{Expert guided and self-guided curricula}\label{expert-G-compare}

Introduced in the above section, the scoring method $s_{E}$ can also be used to guide the learning process in a curriculum learning setting. As the expert model used for scoring share the same network topology as that of the global model that we intend to train and as the expert was trained on the entire dataset, the expert guided curricula can be thought of as a pedagogical mode of learning. 


\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ClientCurr/CC_curr_GisE.eps}
         \caption{Client curriculum}
         \label{subfig:CC_curr_GisE}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ClientCurr/DC_curr_GisE.eps}
         \caption{Data curriculum}
         \label{subfig:DC_curr_GisE}
     \end{subfigure}
    \vspace{-3mm}
\caption{\footnotesize \textbf{To Fill.} To complete.}
\label{fig:GisE_curr}
\end{figure}

\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ClientCurr/CC_anti_GisE.eps}
         \caption{Client curriculum}
         \label{subfig:CC_anti_GisE}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ClientCurr/DC_anti_GisE.eps}
         \caption{Data curriculum}
         \label{subfig:DC_anti_GisE}
     \end{subfigure}
    \vspace{-3mm}
\caption{\footnotesize \textbf{To Fill.} To complete.}
\label{fig:GisE_anti}
\end{figure}

In Fig~\ref{fig:GisE_curr} and Fig~\ref{fig:GisE_anti} we sketch the global model accuracy at different rounds of federation. We see a clear trend in Fig~\ref{fig:GisE_curr} with the $s_{E}$ method outperforming the $s_{G}$ in the initial rounds, but, over the rounds the $s_{G}$ converges to $s_{E}$. Also, the $s_{G}$ accuracy in the initial rounds very closely approximates the random scoring accuracy. 

The $s_{G}$ scoring method is a self-guided curricula, and it uses the global model. In essence the global model is just a random model in the initial rounds of federation and hence the curricula it produces is also random thereby closely approximating the random curricula curve. Overtime as the global model is refined it gets better at determining the "true" curricula thereby converging to the $s_{E}$ curve.

Interestingly, in Fig~\ref{fig:GisE_anti} we find the exact opposite, the $s_{G}$ method outperforming the $s_{E}$ in the initial rounds, but, over the rounds the $s_{E}$ and $s_{G}$ converge. This is in fact a consequence of the very same effect, the $s_{G}$ closely tracks the random curricula in the initial rounds, and random curricula outperforms anti. This is consistent with our observations across experiments. Overtime they tend to converge. These observation corroborate our understanding of global model training process.

This idea of expert guided curricula is interesting to study from an academic view point as it provides critical insights and understanding, but it must be noted that, as the expert model is an oracle expert curricula is not applicable in practice.


\subsection{Ablation study} \label{sec:ablation_study}


\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ClientCurr/Ablation.eps}
         \caption{Client curriculum}
         \label{subfig:CC_w_DC_accuracy_G}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ClientCurr/.eps}
         \caption{Data curriculum}
         \label{subfig:CC_w_DC_accuracy_E}
     \end{subfigure}
    \vspace{-3mm}
\caption{\footnotesize \textbf{To Fill.} To complete.}
\label{fig:CC_w_DC_accuracy}
\end{figure}



In this section, we study the interplay between the data curriculum and the client curriculum, and measure their contributions towards the global model accuracy and the rate of learning. As reported in Fig~\ref{fig:CC_w_DC_accuracy}, we observe that the client curriculum and the data curriculum independently outperform the baseline by \textcolor{red}{XX}\% and \textcolor{red}{XX}\% respectively. In addition, we observe a synergic effect of the combination that outperforms both the curricula, and the baseline by \textcolor{red}{XX}\%. 

We also observe a similar synergy in the rate of learning, see Fig~\ref{fig:CC_w_DC_roc_E} and Fig~\ref{fig:CC_w_DC_roc_G}. 




==> draft.tex <==
\section{Introduction}
\label{sec:intro}




Inspired by the learning principle underlying the cognitive process of humans, curriculum learning (CL) generally proposes to initiate training models with easier aspects of a task, and then gradually move to more complex instances. Prior empirical studies has demonstrated that CL is effective in avoiding bad local minima and in improving the generalization result~\cite{}. In contrast, another line of works proposed opposing strategies emphasizing harder examples, such as anti-curriculum~\cite{}, showing improved results compared to CL in certain scenarios. That can be a reason explaining why this training paradigm (CL) has not been widely adopted in mainstream works. In other contexts such as object detection~\cite{}, and large-scale text models~\cite{}, however, CL is a standard practice. A recent work~\cite{} tried to address the aforementioned contradictory empirical observations to clarify the under what condition CL is useful. In a systematic attempt they conclude that first, the order in which instances are learned is consistent across runs, and similar architectures, also well-known notions of sample difﬁculty are highly correlated with each other, second, curriculum learning, random, and anti-curriculum learning perform almost equally in the standard centralized training, third, CL performs better than the standard centralized training when training time is limited. 


scholars have been exploiting its power in considerably wide application

wide application scopes, including supervised learning tasks within computer vision (CV) [31], [40], natural language processing (NLP) [86], [112], healthcare prediction [14], etc., various reinforcement learning (RL) tasks [20], [77], [93] as well as other applications such as graph learning [25], [88] and neural architecture search (NAS) [32]. The advantages of applying CL training strategies to miscellaneous real-world



However, to the best of our knowledge, little effort has been made to systematically summarize the methodologies and applications of CL.

In this paper, we ﬁll this gap by comprehensively reviewing CL and summarizing its methodologies. To be more


This study motivated us to investigate the 


This work is an attempt to improve our understanding of curricula systematically. We start by asking a very fundamental question about a phenomenon that we call implicit curricula. Are examples



SPCL represents a general learning paradigm that combines the merits from both the CL and SPL.






\textbf{Contributions:} In this paper, in an comprehensive study we investigate for the first time the usage of Curriculum Learning (CL) in FL to boost the classiﬁcation accuracy performance. 

Our CL approach is implemented via a data scheduler, which establishes a prioritization of the training samples. We assign higher importance to samples that are forgotten after the deployment of the global model. We show that presenting the training samples in this order is beneﬁcial for FL, and also boosts the domain alignment between domain pairs. Similar to [8] we employ federated adversarial learning [2], [9] to deal with the alignment between the different domains. However, unlike Li et al. [8] that analyze 1-D signals extracted from fMRI, we study the screening of high-resolution mammograms and use CL to boost the classiﬁcation performance. We validate our strategy on a setup composed of one public and two private clinical datasets with non-IID intensity distributions. Different from [10], who proposes a FL framework for breast density classiﬁcation and do not correct the misalignment between the domains, we target the more complex task of breast cancer classiﬁcation. Furthermore, we propose a novel curriculum for the FL setting, and explicitly handle domain shift with federated adversarial domain adaptation.






\section{My points}
\begin{itemize}
    \item we cover IID and Non-IID
    \item our study also covers CL in few shot. because in FL the clients data are a few.
    \item In CL, the curriculum is assumed to be given by an oracle beforehand, and remains ﬁxed thereafter. In SPL, the curriculum is dynamically generated by the learner itself, according to what the learner has already learned.
    \item Its drawback stems from the fact that the curriculum design is determined independently of the subsequent learning, which may result in inconsistency between the ﬁxed curriculum and the dynamically learned models. From the optimization perspective, since the learning proceeds iteratively, there is no guarantee that the predetermined curriculum can even lead to a converged solution.
    
    
    
\end{itemize}


==> draft2.tex <==

 - Practical Federated Learning setting is In-situ 
 
A major appeal of federated learning is in its ability to enable training of a model in a decentralised manner, which obviates the need for collating the data into a centralized location. In the real-world, the distributed dataset is often generated in-situ at the federating client and the data is measured/generated using a particular sensor belonging to the client. For example, consider the case of a 
 
Consider a real-world scenario of users that participate in federated learning, in which, the users bring along with them their locally stored data that is often sourced/generated/collected on the same device that participates in the federation. For example a smartphone camera device that brings along the photographs taken by the very same device for federation. As there is a huge diversity in the make and quality of smartphone cameras we have a wide spectrum of quality in images, also these devices/sensors could have idiosyncratic distortions and noise in the data they produce. This creates a heterogeneous user base with a wide gamut of data quality. Interestingly, as these effects apply consistent to all the data at a specific user, the relative quality of data is quite consistent in the local user dataset.  

In the previous sections, we have studied the effects of curriculum in the Federated learning setting. In this section, we will look into certain federated learning scenarios in which curriculum does not work.

The heterogeneity in the quality of the user datasets and their relative local consistency naturally translates into an ordering over the datasets (thereby users) of varying difficulty, the data of which is of relatively consistent difficulty. (Prove this). The difficulty of a a dataset/user is quantified by the mean of loss and the consistency is quantified by the variance of loss of the constituent data points. 

Curriculum on Federated Learning behaves very differently in such a scenario. 

For the experiments in this section, we require dataset partitions of varying difficulty and different levels of non-iidness. The task of generating this dataset entails two challenges, one, accurately determine the difficulty of the data points, two, partitioning the data at the desired difficulty level and non-iidness. In order to address the first challenge, we use an apriori trained expert model $\theta_{\mathcal{E}}$ of the same network topology as that of the global model, which is the model of interest, for ranking the data points. As the expert is of the same kind of network and is pretrained on the entire training set it is an accurate judge of the difficulty of the data points. For the second challenge, we first partition the global dataset into the desired non-iid partitions and then we attempt to reshuffle the data among partitions in an increasing order of difficulty while honoring the non-iid class counts of each of the partitions as determined by the non-iid distribution (See Algorithm~\ref{alg:partiiton_diff_dist}).

==> global-personalized.tex <==
% \subsection{Which baselines benefit most from CL?}


% \subsubsection{Under IID}

